Incentive-aware Contextual Pricing with Non-parametric Market Noise

We consider a dynamic pricing problem for repeated contextual second-price auctions with multiple strategic buyers who aim to maximize their long-term time discounted utility. The seller has limited information on buyers' overall demand curves which depends on a non-parametric market-noise distribution, and buyers may potentially submit corrupted bids (relative to true valuations) to manipulate the seller's pricing policy for more favorable reserve prices in the future. We focus on designing the seller's learning policy to set contextual reserve prices where the seller's goal is to minimize regret compared to the revenue of a benchmark clairvoyant policy that has full information of buyers' demand. We propose a policy with a phased-structure that incorporates randomized "isolation" periods, during which a buyer is randomly chosen to solely participate in the auction. We show that this design allows the seller to control the number of periods in which buyers significantly corrupt their bids. We then prove that our policy enjoys a $T$-period regret of $\widetilde{\mathcal{O}}(\sqrt{T})$ facing strategic buyers. Finally, we conduct numerical simulations to compare our proposed algorithm to standard pricing policies. Our numerical results show that our algorithm outperforms these policies under various buyer bidding behavior.

==> 04_fullinfo.tex <==
\section{Truthful Setting: NPAC-T Policy} \label{Sec:fullinfo}
\vspace{-2mm}
In this section, we study the problem of learning contextual reserve prices in the setting where all buyers are truthful and bid their true valuations, i.e. $b_{i,t} = v_{i,t}$ for any $ i\in[N]$ and $t\in[T]$. Hence, here  we will use the terms ``bids'' and ``valuations'' interchangeably. Recall that  the seller observes bids of all the $N$ buyers in each period. To design a pricing policy under this setting, we need to learn the mean vector $\beta$ and the noise  distribution $F$ simultaneously. 
 For the purpose of motivating our policy design, suppose that the mean vector $\beta$ is known to the seller. Recall that, conditioned on $x_t$,  $F^+$ and $F^-$ are respectively  the  distributions of $\epsilon_t^+ = v_t^+ - \langle \beta, x_t \rangle$ and $\epsilon_t^- = v_t^- - \langle \beta, x_t \rangle$. Therefore, one can naturally estimate $F^+$ and $F^-$ via constructing their corresponding empirical distributions using the highest and second-highest bids and knowledge of the mean vector $\beta$. More specifically, in period $t \in[T]$, one can construct the  most up-to-date empirical distributions \[
 \widehat{F}_t^+({z}) =\frac{1}{t-1}\cdot \sum_{\tau \in [t-1]} \I\{v_t^+ - \langle \beta, x_t \rangle \leq {z} \} ~~\text{and}~~
 \widehat{F}_t^-({z})= \frac{1}{t-1}\cdot\sum_{\tau \in [t-1]} \I\{v_t^- - \langle \beta, x_t \rangle \leq {z} \}\,,
 \] and use these estimates as surrogates for $F^+$ and $F^-$ respectively in Equation (\ref{eq:opt_reserve}) to obtain an approximation of the optimal reserve price. However, one of the  main challenges is that the mean  vector $\beta$ is unknown, and as a result, to get any estimate of $F^+$ and $F^-$, we would need to replace $\beta$ in the empirical distributions (particularly within the indicator functions) with some estimate $\widehat{\beta}$, whose estimation error could then potentially propagate into the estimation errors in distributions $F^+$ and $F^-$. We will later discuss how we resolve this error propagation issue. We highlight that because distribution $F$ is non-parametric, a joint estimation of the distributions and  mean vector via a maximum likelihood estimator is not possible. Yet, despite the challenges that arise from embedding the estimate for $\beta$ in the estimates for $F^+$ and $F^-$, this intuition provides a rather straightforward direction to design our pricing policy, named NPAC-T: The policy sequentially  estimates $\beta$, $F^-$,  and $F^+$ as more data points are observed, and uses its most recent estimate of $\beta$ and $F^-$,  and $F^+$ to set reserve prices. Let $\widehat{\beta}_t$ be the  estimate of the mean vector $\beta$  and $\widehat{F}_{t}^-(\cdot)$, $\widehat{F}_{t}^+(\cdot)$  be  the  estimates of $F^{+}(\cdot)$ and $F^-(\cdot)$ respectively, at the beginning of period $t$. (We will define these estimates in the next paragraph.) Then, inspired by the optimal reserve price stated in Equation (\ref{eq:opt_reserve}), the policy sets the reserve price $r_t$ by replacing $\beta$, $F^-$,  and $F^+$ with their estimates, as shown in  Equation (\ref{eq:reserve_price_1}). 
% \negin{Remove this please ``Here, we note that the interval $(0,v_{\max}]$ in  (\ref{eq:reserve_price_1}) determines the ``feasible region" for the reserve price in period $t$, in contrast with the feasible region $[0,\infty)$ in Equation (\ref{eq:opt_reserve}). This is because the  optimal contextual reserve price $r_t^\star(x_t)$ lies in the interval $(0,v_{\max}]$ almost surely and hence in order to approximate this optimal contextual reserve it suffices for the seller to set a reserve price that is at most $v_{\max}$."} 


We now proceed to describe our estimation procedures. In any period $t\in [T]$, we use the average of submitted bids across all the previous periods,  i.e.,  $\bar v_{\tau}  = (\sum_{i\in [N]} v_{i, \tau})/N$ for any  $\tau \in [t-1]$,  to estimate the mean vector using an Ordinary Least Squares (OLS) estimator. Our estimate of $\beta$ at the beginning of period $t$---before the auction is run---is denoted by  $\widehat \beta_{t}$ and  is given in Equation (\ref{eq:fullinfobetaestimate}). In Equation (\ref{eq:fullinfobetaestimate}), $A^\dag$ represents the pseudo inverse of a matrix $A$, so if $A$ is invertible,  we have $A^\dag = A^{-1}$.\footnote{In Lemma \ref{lemma:full:bias}, we show that with high probability, $\sum_{\tau \in [t-1]} x_\tau x_\tau^\top$ in Equation (\ref{eq:fullinfobetaestimate}) is positive definite, and hence invertible.} We then use the most recent estimate of $\beta$, i.e., $\widehat{\beta}_t$, to update our estimate of $F^+$ and $F^-$; see  Equation (\ref{eq:fullinfoalgoFestimate}). We also note that the policy does not require any pure exploration periods. The reason is that at the end of each auction,  all bids are revealed to the seller and as a result, the seller can evaluate the revenue that he could have obtained had he posted any other reserve price other than $r_t$.


\begin{algorithm}
\begin{center}
\footnotesize{
\parbox{\columnwidth}{
%\State 
\textbf{Initialize}: $\widehat{\beta}_1 = 0$,  and $\widehat{F}_1^-(z) =\widehat{F}_1^+(z) = 0$ for $\forall z \in \R$.\\
%\State 
For $t\ge 1$, observe $x_t\sim \mathcal{D}$. Then, \begin{itemize}
        \item [-] \textbf{Set reserve price:}
    \begin{align} 
    \label{eq:reserve_price_1}
     r_t = \arg\max_{y\in [0, v_{\max}]}   \left\{ 
        \int_{0}^y \widehat F^{-}_t\left(z- \langle \widehat\beta_t,x_t \rangle \right)dz - y \left( \widehat F^{+}_t(y- \langle \widehat \beta_t,x_t \rangle)\right)\right\}\,.
    \end{align}
    \item [-] \textbf{Update the estimate of the mean vector:}  %$\widehat{\beta}_{t+1} $, $\widehat{F}_{t+1}^-(\theta)$ and $\widehat{F}_{t+1}^+(\theta)$:
    \begin{align} 
    \label{eq:fullinfobetaestimate}
            & \widehat{\beta}_{t+1}  = \Big( \sum_{\tau \in [t]} x_\tau x_\tau^\top \Big)^\dag \Big( \sum_{\tau \in [t]} x_\tau \Bar{v}_\tau   \Big)  ~~~ \text{where}~~~\bar v_{\tau}  = \frac{1}{N} \sum_{i\in [N]} v_{i, \tau}\,.
        \end{align}
       \item [-] \textbf{Update the estimate of $F^+$ and $F^-$:}  For any $z \in \mathbb{R}$, we have
            \begin{align} \label{eq:fullinfoalgoFestimate}
                \widehat{F}_{t+1}^+(z)  =
              \frac{1}{t} \sum_{\tau \in [t]} \I(v_{\tau}^+ - \langle \widehat{\beta}_{t+1}, x_\tau \rangle \leq  z)       ~~~ \text{and}~~~
              \widehat{F}_{t+1}^-(z)  =
               \frac{1}{t} \sum_{\tau \in [t]} \I(v_{\tau}^- - \langle \widehat{\beta}_{t+1}, x_\tau \rangle \leq  z)\,.
        \end{align}
    \end{itemize}
}}
\end{center} 
\vspace{-0.2cm}
\caption{\footnotesize{NPAC-T Policy: Non-Parametric Contextual Policy against Truthful Buyers}}\label{algo:fullinfo}
\end{algorithm}

Here, we briefly address how one can solve the optimization problem in Equation (\ref{eq:reserve_price_1}). The key observation is that for any period $t$, $\widehat{F}_t^+(\cdot)$ is a step function with jumps at points in the finite set $B_t^+:= \{v_{\tau}^+ - \langle \widehat{\beta}_t , x_{\tau}\rangle \}_{\tau\in[t]}$. Furthermore, $\widehat{F}_t^+({z}) = 0$ for any ${z} < \min B_t^+$ and $\widehat{F}_t^+({z}) = 1$ for any ${z}\geq  \max B_t^+$. Similarly, we have a corresponding finite set $B_t^-:= \{v_{\tau}^- - \langle \widehat{\beta}_t , x_{\tau}\rangle \}_{\tau\in[t]}$ which includes all jump points for $\widehat{F}_t^-(\cdot)$. This implies that in order to solve for the optimal reserve price $r_t$ in Equation (\ref{eq:reserve_price_1}), it suffices to conduct a grid search for $\forall {y} \in B_t^+ \cup B_t^-$. More specifically, we let $ \{z^{(0)}, z^{(1)}, \dots z^{(M)}\}$ be the ordered list (in increasing order) of all elements in $B_t^+ \cup B_t^- \cup \{0\}$, where $z^{(0)} := 0$ and $M := |B_t^+ \cup B_t^-|$ (here, we assumed that $0\notin B_t^+ \cup B_t^- $ without loss of generality). Hence,
\begin{align*}
    r_t ~ = ~ &\arg\max_{m \in [M]} \left\{ 
    \sum_{j=1}^m \widehat F^{-}_t\left(z^{(j)} - \langle \widehat\beta_t,x_t \rangle \right)\cdot(z^{(j)} - z^{(j-1)}) - z^{(m)} \left( \widehat F^{+}_t(z^{(m)}- \langle \widehat \beta_t,x_t \rangle)\right)\right\} \,.
\end{align*}
This shows that the complexity to solve Equation (\ref{eq:reserve_price_1}) is $\mathcal{O}(M^2)$. More detailed discussions and efficient algorithms regarding related problems can be found in \cite{mohri2016learning}.

Demonstrating the NPAC-T policy  has good
performances is 
 challenging because estimation errors for $\beta$ will further propagate into the estimation errors in $F^-$ and $F^+$. Here, we highlight that one cannot naively apply CDF-based concentration inequalities (e.g. the Dvoretzky-Kiefer-Wolfowitz Inequality) to bound the distribution estimation errors. This is because the estimates $\widehat{F}_t^+(\cdot) $ and $\widehat{F}_t^-(\cdot)$ evaluated at any point ${z} \in\R$ are biased. To see why, note that because of the estimation error in the mean vector $\beta$, the terms $v_{\tau}^+ - \langle \widehat{\beta}_{t+1},x_\tau \rangle $ and $v_{\tau}^- - \langle \widehat{\beta}_{t+1}, x_\tau \rangle $ in the expressions for $\widehat{F}_t^+(\cdot) $ and $\widehat{F}_t^-(\cdot)$ are not realizations of $\epsilon_\tau^-$ and $\epsilon_\tau^+$, respectively. In particular, $\expect\left[\widehat{F}^{-}_t\big(z- \langle \widehat\beta_t,x_t \rangle \big)\right] \neq F\big(z- \langle \widehat{\beta_t},x_t \rangle \big)$. This also sheds light on the more subtle and challenging issue:  the estimates $\widehat{F}_t^+(\cdot) $ and $\widehat{F}_t^-(\cdot)$ are evaluated at points which may be random variables that  depend on all information up to time $t$. Observe that the expression $F^-\big(z- \langle \widehat{\beta_t},x_t \rangle \big)$ is itself a random variable since $\widehat{\beta_t}$ depends on the entire past history up to the current period. The same issue occurs when bounding the error for $\widehat{F}_t^+(\cdot) $. Nevertheless, the following Lemma \ref{lemma:full:estimateF} demonstrates that we are still able to provide good estimation error guarantees for the distributions.

\begin{lemma}[Bounding Estimation Errors in $F^-$ and $F^+$] \label{lemma:full:estimateF} {Define $\sigma_t$ to be the sigma algebra generated by all $\{x_\tau\}_{\tau \in[t]} $ and $\{\epsilon_{i,\tau}\}_{i\in [N],\tau \in[t]} $.}  Then, for any $\sigma_t$-measurable random variable ${z}$ and any $\gamma> 0$, we have 
\begin{align*}
    \prob\left( \left|F^-(z)-  \widehat{F}_t^-(z) \right| \leq \gamma + 2c_f N^2\delta_t \right) ~ \geq ~  1 - 4\exp\left( -t\gamma^2\right) - \frac{4d}{(t-1)^2}-  2d\exp\left( -\frac{(t-1)\lambda_0^2}{8x_{\max}^2}\right)\, \text{ and}
\end{align*}
\begin{align*}
    \prob\left( \left|F^+(z)-  \widehat{F}_t^+(z) \right| \leq \gamma + c_f N\delta_t \right) ~ \geq ~  1 - 4\exp\left( -t\gamma^2\right) - \frac{4d}{(t-1)^2}-  2d\exp\left( -\frac{(t-1)\lambda_0^2}{8x_{\max}^2}\right)\,,
\end{align*}
{where $\delta_{t} = \frac{4\sqrt{d\log(t-1)}\epsilon_{\max} x_{\max}^2}{\lambda_0^2\sqrt{N(t-1)}}$, $c_f = \sup_{{z}\in [-\epsilon_{\max},\epsilon_{\max}]}f(z)$, and $\lambda_0^2 > 0$ is the smallest eigenvalue of $\Sigma = \expect_{x\sim\mathcal{D}}[xx^T]$.}
\end{lemma}
The key idea to prove this lemma, or in other words to bound the estimation error $|F^-(z)-  \widehat{F}_t^-(z) |$ and $|F^+(z)-  \widehat{F}_t^+(z) |$ for any ${z}\in \R$, is to first control for the estimation errors in $\beta$, i.e. by assuming that our estimation error for $\beta$ is small, namely $\norm{\widehat{\beta}_t - \beta}_1 \leq \delta_t/x_{\max}$. Then, we rely on the Lipschitz properties for the distributions $F$, $F^-$ and $F^+$, which are shown in Lemma \ref{lemma:FF-F+Lipschitz} of Appendix \ref{appsec:truthfullotherlem}, to separate the estimation errors in $\beta$ from those of the distributions. After this ``separation procedure'', we can then return to applying distributional concentration inequalities. The detailed proof of Lemma \ref{lemma:full:estimateF} can be found in Appendix \ref{appsec:truthfulllem}. Note that the term $\delta_t=\mathcal{O}(\sqrt{\log(t)/(Nt)})$ in the bounds for $|F^-(z)-  \widehat{F}_t^-(z) |$ and $|F^+(z)-  \widehat{F}_t^+(z) |$ can be viewed as the estimation error for $\beta$, which echoes our earlier point that estimation error in the mean vector propagates into the inaccuracy of the distributions' estimates. In Lemma \ref{lemma:full:bias} of Appendix \ref{appsec:truthfullotherlem}, we show  $\norm{\widehat{\beta}_t - \beta}_1 \leq \delta_t/x_{\max}$ occurs with high probability.

Finally, the following theorem is the main result of this section and upper bounds the regret of the NPAC-T policy in the truthful setting.


\begin{theorem}[Regret of NPAC-T Policy]\label{bound:fullInfoRegret}
    Consider the case of $N\geq 2$ buyers. Then, in the truthful setting, the T-period regret of the NPAC-T policy is in the order of $\mathcal{O}\left(c_f\sqrt{dN^3 T\log(T)}\right)$, where the regret is computed against the benchmark in Definition \ref{def:benchmark_policy} that knows the mean vector $\beta$ and noise distribution $F$. Here, $c_f = \sup_{z \in [-\epsilon_{\max}, \epsilon_{\max}]} f(z)> 0$ where $f$ is the the probability density function  of the market noise distribution $F$.
\end{theorem} 

The dependency on $c_f$ in the regret bound of Theorem \ref{bound:fullInfoRegret} indicates estimation accuracy depends on the specific problem instance with respect to the market noise distribution $F$. Here, we point out that the regret bound deteriorates as the market noise instance is more difficult to learn, i.e., when the probability density is rather concentrated in various regions on the real line. %\new{(Delete this sentence) This is the case because, with less concentrated noise probability density functions, each  sample will provide a decent amount of information for other samples (consider a discrete distribution function with only one possible value such that one single sample of the market noise reveals the values of all other market noise variables), but on the other hand, for probability density functions that are abnormally concentrated in certain regions, individual samples will convey less information about other independent market noise realizations.}
{The dependency on $N$ (i.e. the factor $\mathcal{O}\left(N^{{3}/{2}} \right)$) is due to the Lipschitz properties of $F, F^-$ and $F^+$ which are induced by the boundedness of the pdf $f$, as illustrated in Lemma \ref{lemma:FF-F+Lipschitz}.  That is,  if it is directly assumed that distributions $F, F^-$ and $F^+$ satisfy some Lipschitz conditions (that do not depend on $N$), we can improve the regret of the NPAC-T policy to $\mathcal{O}\left({c_f\sqrt{dT\log(T)}}/{\sqrt{N}}\right)$. }


The detailed proof of Theorem \ref{bound:fullInfoRegret} is presented in Appendix \ref{appsec:fullinforoadmap}, and here, we provide an outline for our analysis to upper bound the regret of the NPAC-T policy.

\paragraph{Proof sketch of Theorem \ref{bound:fullInfoRegret}}  We first decompose the single period regret into the revenue loss due to estimation errors for $\beta$, $F^-$ and $F^+$, and hence, the proof boils down to bounding these errors. First, Lemma \ref{lemma:full:bias} in Appendix \ref{appsec:truthfullotherlem} shows that $\norm{\widehat{\beta}_t - \beta}_1 \leq \delta_t/x_{\max}$ with high probability,  where we recall $\delta_t = \mathcal{O}(\sqrt{\log(t)/(Nt)})$. 
%  which indicates the estimation error in $\beta$ decreases as more data points are collected
 Next, by letting $\gamma = \gamma_t = \mathcal{O}(\sqrt{\log(t)/t})$ in Lemma \ref{lemma:full:estimateF}, we see that the estimation errors in $ \widehat{F}_t^-$ and $\widehat{F}_t^+$ are bounded by $\gamma_t + 2c_f N^2 \delta_t =  \mathcal{O}(c_{f}\sqrt{N^3\log(t)/t})$ and $\gamma_t + c_f N \delta_t = \mathcal{O}(c_{f}\sqrt{N\log(t)/t})$ with high probability, respectively. Finally, combining these results, we sum up the cumulative single period revenue losses to attain the cumulative expected regret for the NPAC-T policy.
 
 
 
%  (e.g. $z = r_t - \langle \widehat{\beta}_t, x_\tau \rangle$ for some $\tau < t$, where both $r_t$ and $\widehat{\beta}_t$ are measurable functions of $\mathcal H_t^F$. 
%  as there are difficulties in finding the expectations of $\widehat{F}_t^-(z)$ and $\widehat{F}_t^+(z)$, given the fact that 
 
 

 
 

















==> 08_conclusion.tex <==
\section{Concluding Remarks} 
\label{Sec:conclusion}

The problem of designing data-driven optimal auctions has drawn much attention lately; see, for example, \cite{roughgarden2016minimizing, golrezaei2017boosted, derakhshan2019lp}, and \cite{javanmard2016dynamic}. There, the goal is to deviate from classical Bayesian settings and take advantage of available data to optimize auction design either in an offline or online fashion. Although this approach is very natural, it can lead to designs that are vulnerable to buyers' manipulations as the data may be generated by strategic buyers. In this work, we show how one can make data-driven auction design robust to buyers' manipulations even in a setting with a contextual and non-parametric demand model. To robustify our data-driven auction design,  
we (i)  restart our policy over time in a systematic way and  (ii)  incorporate randomized isolation periods.  While the former reduces the impact of corrupted (manipulative) bids, the latter makes manipulations costly for the buyers and incentivizes them to well-behave.   
